Row and column detection complexities of character tables

Character tables of finite groups and closely related commutative algebras have been investigated recently using new perspectives arising from the AdS/CFT correspondence and low-dimensional topological quantum field theories. Two important elements in these new perspectives are physically motivated definitions of quantum complexity for the algebras and a notion of row-column duality. These elements are encoded in properties of the character table of a group G and the associated algebras, notably the centre of the group algebra and the fusion algebra of irreducible representations of the group. Motivated by these developments, we define row and column versions of detection complexities for character tables, and investigate the relation between these complexities under the exchange of rows and columns. We observe regularities that arise in the statistical averages over small character tables and propose corresponding conjectures for arbitrarily large character tables.

==> tikzlibrarytqft.code.tex <==
%%
%% This is file `tikzlibrarytqft.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tqft_code.dtx  (with options: `library')
%% ----------------------------------------------------------------
%% tqft --- a TikZ library for drawing TQFT diagrams
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\ProvidesFile{tikzlibrarytqft.code.tex}[2024/05/31 v2.3 Tikz/PGF commands for drawing TQFT diagrams]
\ifcsname pgfk@/handlers/.pic/.@cmd\endcsname
\else
\pgfwarning{This library only works with TikZ 3.0 or later; for earlier versions of TikZ use the TQFT package}
\fi
\usetikzlibrary{shapes.geometric}
\def\pgf@tqft@minus{-}
\let\pgf@tqft@upper\@empty
\let\pgf@tqft@lower\pgf@tqft@minus
\newif\iftqft@twisted
\def\tqft@split(#1,#2){%
  \pgfmathsetmacro\tqft@y{#2 * (-\tqft@val{cobordism height})}%
  \pgfmathsetmacro\tqft@x{(#1 - 1 + max(min(#2,1),0)*\tqft@val{offset}) * \tqft@val{boundary separation}}%
  \def\tqft@shift{(\tqft@x pt, \tqft@y pt)}%
}%
\tikzset{
    pic alias/.code={%
      \tikz@fig@mustbenamed
      \expandafter\def\expandafter\tikz@alias\expandafter{\tikz@alias\pgfnodealias{\tikz@pp@name{#1}}{\tikz@fig@name}}%
    },
  tqft/.style={%
    pic type=cobordism,
    every tqft/.try,
    tqft/.cd,
  },
  tqft/.unknown/.code={%
    \let\tqft@searchname=\pgfkeyscurrentname%
    \pgfkeysalso{%
      /tikz/\tqft@searchname={#1}
    }
  },
  tqft/.cd,
  incoming boundary components/.initial=5,
  outgoing boundary components/.initial=4,
  skip incoming boundary components/.initial={},
  skip outgoing boundary components/.initial={},
  genus/.initial = 0,
  offset/.initial=0,
  cobordism height/.initial=2cm,
  boundary separation/.initial=2cm,
  circle x radius/.initial=10pt,
  circle y radius/.initial=5pt,
  view from/.is choice,
  view from/incoming/.code={%
    \let\pgf@tqft@upper\pgf@tqft@minus
    \let\pgf@tqft@lower\@empty
  },
  view from/outgoing/.code={%
  \let\pgf@tqft@lower\pgf@tqft@minus
    \let\pgf@tqft@upper\@empty
  },
  twisted/.is if=tqft@twisted,
  anchor/.initial = none,
  pair of pants/.style={
    /tikz/tqft,
    incoming boundary components=1,
    outgoing boundary components=2,
    offset=-.5
  },
  /tikz/tqft pair of pants/.style={
    /tikz/tqft/pair of pants,
  },
  reverse pair of pants/.style={
    /tikz/tqft,
    incoming boundary components=2,
    outgoing boundary components=1,
    offset=.5
  },
  /tikz/tqft reverse pair of pants/.style={
    /tikz/tqft/reverse pair of pants,
  },
  cylinder to prior/.style={
    /tikz/tqft,
    incoming boundary components=1,
    outgoing boundary components=1,
    offset=-.5
  },
  /tikz/tqft cylinder to prior/.style={
    /tikz/tqft/cylinder to prior,
  },
  cylinder to next/.style={
    /tikz/tqft,
    incoming boundary components=1,
    outgoing boundary components=1,
    offset=.5
  },
  /tikz/tqft cylinder to next/.style={
    /tikz/tqft/cylinder to next,
  },
  cylinder/.style={
    /tikz/tqft,
    incoming boundary components=1,
    outgoing boundary components=1
  },
  /tikz/tqft cylinder/.style={
    /tikz/tqft/cylinder,
  },
  cup/.style={
    /tikz/tqft,
    incoming boundary components=1,
    outgoing boundary components=0
  },
  /tikz/tqft cup/.style={
    /tikz/tqft/cup,
  },
  cap/.style={
    /tikz/tqft,
    incoming boundary components=0,
    outgoing boundary components=1
  },
  /tikz/tqft cap/.style={
    /tikz/tqft/cap,
  },
}
\def\tqft@val#1{\pgfkeysvalueof{/tikz/tqft/#1}}
\tikzset{
  cobordism/.pic={
      \gdef\tqft@fullpath{}%
      \global\let\tqft@blist\pgfutil@gobble%
      \gdef\tqft@gclip{}%
      \global\let\tqft@glist\pgfutil@gobble%
      \global\let\tqft@clist\pgfutil@gobble%
      \global\let\tqft@alist\pgfutil@gobble
      \global\let\tqft@ibdrylist=\pgfutil@gobble
      \global\let\tqft@cibdrylist=\pgfutil@gobble
      \global\let\tqft@obdrylist=\pgfutil@gobble
      \global\let\tqft@cobdrylist=\pgfutil@gobble
      \global\let\tqft@robdrylist=\pgfutil@gobble
      \global\let\tqft@rcobdrylist=\pgfutil@gobble
    \iftqft@twisted
    \pgfmathsetmacro\tqft@outgoing@end{0}%
    \pgfmathsetmacro\tqft@outgoing@dir{-1}%
    \else
    \pgfmathsetmacro\tqft@outgoing@end{1}%
    \pgfmathsetmacro\tqft@outgoing@dir{1}%
    \fi
      \ifnum\tqft@val{incoming boundary components}>0\relax
      \xdef\tqft@fullpath{%
        \tqft@fullpath
        (-\tqft@val{circle x radius},0) arc[start angle=\pgf@tqft@upper180, end angle=0, x radius=\tqft@val{circle x radius}, y radius=\tqft@val{circle y radius}]
      }%
      \xdef\tqft@alist{%
        \tqft@alist,-incoming boundary 1/{(0,0)},-incoming boundary/{(0,0)}%
      }%
    \ifnum\tqft@val{incoming boundary components}>1\relax
    \foreach \k in {2,...,\tqft@val{incoming boundary components}} {
      \edef\tqft@temp{\noexpand\pgfutil@in@{,\k,}{,\tqft@val{skip incoming boundary components},}}
      \tqft@temp
      \ifpgfutil@in@
      \xdef\tqft@cibdrylist{\tqft@cibdrylist,\k}
      \else
      \xdef\tqft@ibdrylist{\tqft@ibdrylist,\k}
      \fi
    }
    \ifx\tqft@ibdrylist\pgfutil@gobble
    \else
    \foreach \k [
      remember=\k as \kmo (initially 1),
        evaluate=\k as \xpos using (\k-1)*\tqft@val{boundary separation} -\tqft@val{circle x radius},
    ] in \tqft@ibdrylist {
      \pgfmathsetmacro\xppos{(\kmo - 1)*\tqft@val{boundary separation} + \tqft@val{circle x radius}}
      \pgfmathsetmacro\cpos{(\xpos + \xppos)/2}
        \xdef\tqft@fullpath{%
          \tqft@fullpath
           .. controls +(0,-\tqft@val{cobordism height}/3) and +(0,-\tqft@val{cobordism height}/3) ..  (\xpos pt,0) arc[start angle=\pgf@tqft@upper180, end angle=0, x radius=\tqft@val{circle x radius}, y radius=\tqft@val{circle y radius}]
      }%
        \xdef\tqft@blist{%
          \tqft@blist,incoming boundary \k/incoming/{%
      (\xppos pt,0) .. controls +(0,-\tqft@val{cobordism height}/3) and +(0,-\tqft@val{cobordism height}/3) .. (\xpos pt,0)}%
      }%
      \xdef\tqft@clist{%
        \tqft@clist,-between incoming \kmo\space and \k/{(\cpos pt,-\tqft@val{cobordism height}/4)}%
      }%
      \xdef\tqft@alist{%
        \tqft@alist,-incoming boundary \k/{(\kmo * \tqft@val{boundary separation},0)}%
      }%
    }%
    \fi
      \fi
      \ifnum\tqft@val{outgoing boundary components}>0\relax
    \pgfmathsetmacro\xppos{%
      (\tqft@outgoing@end * (\tqft@val{outgoing boundary components} -1)
      + \tqft@val{offset}) * \tqft@val{boundary separation}
      + \tqft@outgoing@dir * \tqft@val{circle x radius}}%
      \pgfmathsetmacro\tqft@ht{abs(\tqft@val{incoming boundary components} - \tqft@val{outgoing boundary components} - \tqft@val{offset})}%
      \pgfmathsetmacro\tqft@ht{1/3 + 2/3*\tqft@ht/(\tqft@ht + 1)}%
      \xdef\tqft@fullpath{%
        \tqft@fullpath
        .. controls +(0,-\tqft@ht*\tqft@val{cobordism height}) and +(0,\tqft@ht*\tqft@val{cobordism height}) .. (\xppos pt, -\tqft@val{cobordism height})
      }%
      \xdef\tqft@blist{%
        \tqft@blist,between last incoming and last outgoing/incoming and outgoing/{%
        (\tqft@val{incoming boundary components} * \tqft@val{boundary separation} + \tqft@val{circle x radius} - \tqft@val{boundary separation},0pt)
        .. controls +(0,-\tqft@ht*\tqft@val{cobordism height}) and +(0,\tqft@ht*\tqft@val{cobordism height}) .. (\xppos pt, -\tqft@val{cobordism height})}%
      }%
      \pgfmathsetmacro\xppos{(\xppos + (\tqft@val{incoming boundary components} -1) * \tqft@val{boundary separation} +\tqft@val{circle x radius})/2}%
      \xdef\tqft@clist{%
        \tqft@clist,-between last incoming and last outgoing/{(\xppos pt,-\tqft@val{cobordism height}/2)}%
      }%
      \else
      \pgfmathsetmacro\tqft@ht{1/3 + 2/3*(\tqft@val{incoming boundary components} - 1)/\tqft@val{incoming boundary components}}
      \xdef\tqft@fullpath{%
        \tqft@fullpath
        .. controls +(0,-\tqft@ht*\tqft@val{cobordism height}) and +(0,-\tqft@ht*\tqft@val{cobordism height}) .. (-\tqft@val{circle x radius},0)
      }%
      \xdef\tqft@blist{%
        \tqft@blist,between first and last incoming/incoming and outgoing/{%
        (\tqft@val{incoming boundary components} * \tqft@val{boundary separation} + \tqft@val{circle x radius} - \tqft@val{boundary separation},0pt)
        .. controls +(0,-\tqft@ht*\tqft@val{cobordism height}) and +(0,-\tqft@ht*\tqft@val{cobordism height}) .. (-\tqft@val{circle x radius},0)}
      }%
      \pgfmathsetmacro\xppos{(\tqft@val{incoming boundary components} -1) * \tqft@val{boundary separation}/2}%
      \xdef\tqft@clist{%
        \tqft@clist,-between first and last incoming/{(\xppos pt,-\tqft@ht*\tqft@val{cobordism height}*3/4)},-between first incoming and last incoming/{(\xppos pt,-\tqft@ht*\tqft@val{cobordism height}*3/4)}%
      }%
      \fi
      \else
      \ifnum\tqft@val{outgoing boundary components}>0\relax
        \pgfmathsetmacro\xppos{( \tqft@outgoing@end * (\tqft@val{outgoing boundary components} -1)+\tqft@val{offset}) * \tqft@val{boundary separation} + \tqft@outgoing@dir * \tqft@val{circle x radius}}
      \xdef\tqft@fullpath{%
        \tqft@fullpath
        (\xppos pt, -\tqft@val{cobordism height})
      }%
      \fi
      \fi
    \ifnum\tqft@val{outgoing boundary components}>0\relax
    \pgfmathsetmacro\xppos{%
      ( \tqft@outgoing@end * (\tqft@val{outgoing boundary components} -1)
      + \tqft@val{offset}) * \tqft@val{boundary separation}
      - \tqft@outgoing@dir * \tqft@val{circle x radius}}%
      \xdef\tqft@fullpath{%
        \tqft@fullpath
        arc[end angle=\pgf@tqft@upper180, start angle=0, x radius=\tqft@outgoing@dir * \tqft@val{circle x radius}, y radius=\tqft@val{circle y radius}]
      }%
      \xdef\tqft@alist{%
        \tqft@alist,-outgoing boundary \tqft@val{outgoing boundary components}/{(\xppos pt + \tqft@outgoing@dir * \tqft@val{circle x radius},-\tqft@val{cobordism height})},-outgoing boundary/{(\tqft@val{offset}*\tqft@val{boundary separation},-\tqft@val{cobordism height})}%
      }%
      \ifnum\tqft@val{outgoing boundary components}>1\relax
    \foreach \k [evaluate=\k as \ok using int(\tqft@outgoing@end * (\tqft@val{outgoing boundary components} + 1) - \tqft@outgoing@dir * \k)] in {2,...,\tqft@val{outgoing boundary components}} {
      \edef\tqft@temp{\noexpand\pgfutil@in@{,\ok,}{,\tqft@val{skip outgoing boundary components},}}
      \tqft@temp
      \ifpgfutil@in@
      \xdef\tqft@cobdrylist{\tqft@cobdrylist,\k}
      \else
      \xdef\tqft@obdrylist{\tqft@obdrylist,\k}
      \fi
    }
    \ifx\tqft@obdrylist\pgfutil@gobble
    \else
    \foreach \k [
      remember=\k as \kmo (initially 1),
        evaluate=\k as \xpos using ( \tqft@outgoing@end * (\tqft@val{outgoing boundary components} + 1) - 1 -  \tqft@outgoing@dir * \k + \tqft@val{offset})*\tqft@val{boundary separation} + \tqft@outgoing@dir * \tqft@val{circle x radius},
    ] in \tqft@obdrylist {
      \pgfmathsetmacro\xppos{(\tqft@outgoing@end * (\tqft@val{outgoing boundary components} + 1) - 1 - \tqft@outgoing@dir * \kmo + \tqft@val{offset})*\tqft@val{boundary separation} - \tqft@outgoing@dir * \tqft@val{circle x radius}}
        \pgfmathsetmacro\cpos{(\xpos + \xppos)/2}
        \pgfmathsetmacro\nk{int(\tqft@val{outgoing boundary components} - \k + 1)}
        \pgfmathsetmacro\nkpo{int(\tqft@val{outgoing boundary components} - \kmo + 1)}
        \xdef\tqft@fullpath{%
          \tqft@fullpath
           .. controls +(0,\tqft@val{cobordism height}/3) and +(0,\tqft@val{cobordism height}/3) ..  (\xpos pt,-\tqft@val{cobordism height}) arc[end angle=\pgf@tqft@upper180, start angle=0, x radius=\tqft@outgoing@dir * \tqft@val{circle x radius}, y radius=\tqft@val{circle y radius}]
      }%
        \xdef\tqft@blist{%
          \tqft@blist,between outgoing \nk\space and \nkpo/outgoing/{%
 (\xppos pt,-\tqft@val{cobordism height})
           .. controls +(0,\tqft@val{cobordism height}/3) and +(0,\tqft@val{cobordism height}/3) ..  (\xpos pt,-\tqft@val{cobordism height}) ++(-2*\tqft@val{circle x radius},0)}%
      }%
      \xdef\tqft@clist{%
        \tqft@clist,-between outgoing \nk\space and \nkpo/{(\cpos pt,-3*\tqft@val{cobordism height}/4)}%
      }%
      \xdef\tqft@alist{%
        \tqft@alist,-outgoing boundary \nk/{(\xpos pt - \tqft@val{circle x radius},-\tqft@val{cobordism height})}%
      }%
      }%
    \fi
    \fi
      \ifnum\tqft@val{incoming boundary components}>0\relax
      \pgfmathsetmacro\tqft@ht{1/3 + 2/3*abs(\tqft@val{offset})/(abs(\tqft@val{offset}) + 1)}%
      \xdef\tqft@fullpath{%
        \tqft@fullpath
        .. controls +(0,\tqft@ht*\tqft@val{cobordism height}) and +(0,-\tqft@ht*\tqft@val{cobordism height}) .. (-\tqft@val{circle x radius},0)
      }%
      \xdef\tqft@blist{%
        \tqft@blist,between first incoming and first outgoing/incoming and outgoing/{%
    ({ ( (1 - \tqft@outgoing@end) * (\tqft@val{outgoing boundary components} - 1) + \tqft@val{offset}) * \tqft@val{boundary separation} - \tqft@outgoing@dir * \tqft@val{circle x radius}},-\tqft@val{cobordism height})
        .. controls +(0,\tqft@ht*\tqft@val{cobordism height}) and +(0,-\tqft@ht*\tqft@val{cobordism height}) .. (-\tqft@val{circle x radius},0)}%
      }%
      \xdef\tqft@clist{%
        \tqft@clist,-between first incoming and first outgoing/{({ ( (1 - \tqft@outgoing@end) * (\tqft@val{outgoing boundary components} - 1) +\tqft@val{offset})*\tqft@val{boundary separation}/2- \tqft@outgoing@end * \tqft@val{circle x radius}},-\tqft@val{cobordism height}/2)}%
      }%
      \else
      \pgfmathsetmacro\xppos{(\tqft@val{outgoing boundary components} -1+\tqft@val{offset}) * \tqft@val{boundary separation} +\tqft@val{circle x radius}}%
      \pgfmathsetmacro\tqft@ht{1/3 + 2/3*(\tqft@val{outgoing boundary components} - 1)/\tqft@val{outgoing boundary components}}
      \xdef\tqft@fullpath{%
        \tqft@fullpath
        .. controls +(0,\tqft@ht*\tqft@val{cobordism height}) and +(0,\tqft@ht*\tqft@val{cobordism height}) .. (\xppos pt,-\tqft@val{cobordism height})
      }%
      \xdef\tqft@blist{%
        \tqft@blist,between first and last outgoing/incoming and outgoing/{%
    (\tqft@val{offset} * \tqft@val{boundary separation} - \tqft@val{circle x radius},-\tqft@val{cobordism height})
        .. controls +(0,\tqft@ht*\tqft@val{cobordism height}) and +(0,\tqft@ht*\tqft@val{cobordism height}) .. (\xppos pt,-\tqft@val{cobordism height})}%
      }%
      \pgfmathsetmacro\xppos{(\tqft@val{outgoing boundary components}/2 + \tqft@val{offset} -1/2) * \tqft@val{boundary separation}}%
      \pgfmathsetmacro\tqft@ht{1 -\tqft@ht*3/4}%
      \xdef\tqft@clist{%
        \tqft@clist,-between first and last outgoing/{(\xppos pt,-\tqft@ht*\tqft@val{cobordism height})},-between first outgoing and last outgoing/{(\xppos pt,-\tqft@ht*\tqft@val{cobordism height})}%
      }%
      \fi
      \fi
      \pgfmathsetmacro\xpos{%
        (
        \tqft@val{outgoing boundary components} > 0 ?
        (
        \tqft@val{incoming boundary components} > 0 ?
        min(0,\tqft@val{offset}) : \tqft@val{offset}
        ) : 0
        )
        *\tqft@val{boundary separation} - 2*\tqft@val{circle x radius}}%
      \xdef\tqft@gclip{(\xpos pt,2*\tqft@val{circle y radius}) rectangle }%
      \pgfmathsetmacro\xpos{%
        ((
        \tqft@val{outgoing boundary components} > 0 ?
        (
        \tqft@val{incoming boundary components} > 0 ?
        max(\tqft@val{incoming boundary components},\tqft@val{outgoing boundary components} + \tqft@val{offset}) : \tqft@val{outgoing boundary components} + \tqft@val{offset}
        ) : \tqft@val{incoming boundary components}
        )-1)
        *\tqft@val{boundary separation} + 2*\tqft@val{circle x radius}}%
      \xdef\tqft@gclip{\tqft@gclip (\xpos pt,-\tqft@val{cobordism height} - 2*\tqft@val{circle y radius})}%
      \ifnum\tqft@val{genus}>0\relax
      \pgfmathsetmacro\xpos{%
        (
        \tqft@val{outgoing boundary components} > 0 ?
        (
        \tqft@val{incoming boundary components} > 0 ?
        \tqft@val{offset}/2 : \tqft@val{offset}
        ) : 0
        )
        *\tqft@val{boundary separation} - \tqft@val{circle x radius}}%
      \pgfmathsetmacro\ypos{%
        (
        \tqft@val{outgoing boundary components} > 0 ?
        (
        \tqft@val{incoming boundary components} > 0 ?
        -\tqft@val{cobordism height}/2 : -1 + \tqft@val{cobordism height}/3
        ) : - \tqft@val{cobordism height}/3
        )}%
      \xdef\tqft@gclip{%
        \tqft@gclip
        (\xpos pt,\ypos pt)
      }%
      \pgfmathsetmacro\gsize{%
        ((
        \tqft@val{outgoing boundary components} > 0 ?
        (
        \tqft@val{incoming boundary components} > 0 ?
        (\tqft@val{incoming boundary components} + \tqft@val{outgoing boundary components})/2 : \tqft@val{outgoing boundary components}
        ) : \tqft@val{incoming boundary components}
        )-1)
        *\tqft@val{boundary separation}/\tqft@val{circle x radius} + 2}%
      \pgfmathsetmacro\gscale{min(1,\gsize/(3*\tqft@val{genus}+1))}%
      \pgfmathsetmacro\gyscale{\tqft@val{circle y radius}*\gscale*.707}%
      \pgfmathsetmacro\gxscale{\tqft@val{circle x radius}*\gscale}%
      \pgfmathsetmacro\gsep{((\gsize - 2*\tqft@val{genus}*\gscale)/(\tqft@val{genus} + 1)*\tqft@val{circle x radius}}%
      \xdef\tqft@gclip{%
        \tqft@gclip
        ++(\gsep/2 pt,0)
      }%
      \pgfmathsetmacro\omrstwo{1 - 1/sqrt(2)}%
      \pgfmathsetmacro\sqrtwo{sqrt(2)}%
      \foreach[
        evaluate=\k as \kmo using int(2 * \k-1)
      ] \k in {1,...,\tqft@val{genus}} {
        \xdef\tqft@gclip{%
          \tqft@gclip
          ++(\gsep/2 pt + \omrstwo*\gxscale pt,0)
          .. controls +(\gxscale*\sqrtwo/3 pt,4/3*\gyscale pt) and +(-\gxscale*\sqrtwo/3 pt,4/3*\gyscale pt)
          .. ++(\sqrtwo*\gxscale pt,0)
          .. controls +(-\gxscale*\sqrtwo/3 pt,-4/3*\gyscale pt) and +(\gxscale*\sqrtwo/3 pt,-4/3*\gyscale pt)
          .. ++(-\sqrtwo*\gxscale pt,0)
          ++(2*\gxscale pt -\omrstwo*\gxscale pt + \gsep/2 pt,0)
        }
        \xdef\tqft@glist{%
          \tqft@glist,%
            hole \k/lower/{%
            (\xpos pt + \k * \gsep pt +  \kmo * \gxscale pt + \gxscale pt -\omrstwo*\gxscale pt,\ypos pt)
          .. controls +(-\gxscale pt*\sqrtwo/3,\pgf@tqft@upper4/3*\gyscale pt) and +(\gxscale pt*\sqrtwo/3,\pgf@tqft@upper4/3*\gyscale pt)
          .. ++(-\sqrtwo*\gxscale pt,0)},%
          hole \k/upper/{(\xpos pt + \k * \gsep pt +  \kmo * \gxscale pt - \gxscale pt,\ypos pt + \pgf@tqft@upper\gyscale pt)%
          .. controls +(\gxscale pt*2/3,\pgf@tqft@lower8/3*\gyscale pt) and +(-\gxscale pt*2/3,\pgf@tqft@lower8/3*\gyscale pt)
          .. ++(2*\gxscale pt,0)}%
        }%
        \xdef\tqft@clist{%
          \tqft@clist,-hole \k/{(\xpos pt + \k * \gsep pt +  \kmo * \gxscale pt,\ypos pt)}%
        }%
      }%
      \fi
\gdef\tqft@shift{(0,0)}%
\edef\tqft@anchor{\tqft@val{anchor}}%
\expandafter\pgfutil@in@\expandafter{\expandafter,\expandafter}\expandafter{\tqft@anchor}%
\ifpgfutil@in@
\expandafter\tqft@split\tqft@anchor\relax
\else
\edef\tqft@anchor{-\tqft@val{anchor}}%
\xdef\tqft@alist{\tqft@clist,\tqft@alist}%
\foreach \anchor/\coord in \tqft@alist
{
  \ifx\anchor\tqft@anchor\relax
  \global\let\tqft@shift\coord
  \fi
}%
\fi
\tikz@scan@one@point\pgfutil@firstofone\tqft@shift\relax
\begin{scope}[shift={(-\pgf@x,-\pgf@y)}]
\ifnum\tqft@val{incoming boundary components}>0\relax
\ifx\tqft@ibdrylist\pgfutil@gobble
\xdef\tqft@ibdrylist{1}
\else
\xdef\tqft@ibdrylist{1,\tqft@ibdrylist}
\fi
      \foreach[evaluate=\k as \xpos using (\k-1)*\tqft@val{boundary separation}] \k in \tqft@ibdrylist {
  \node[
    transform shape,
          node contents={},
          ellipse,
          inner sep=0pt,
          outer sep=0pt,
          minimum width=2*\tqft@val{circle x radius},
          minimum height=2*\tqft@val{circle y radius},
          at={(\xpos pt,0)},
          name=-incoming boundary \k,
          /tikz/tqft/every boundary component/.try,
          /tikz/tqft/every incoming boundary component/.try,
          /tikz/tqft/incoming boundary component \k/.try
        ];
      }%
\ifx\tqft@cibdrylist\pgfutil@gobble
\else
      \foreach[evaluate=\k as \xpos using (\k-1)*\tqft@val{boundary separation}] \k in \tqft@cibdrylist {
  \node[
    transform shape,
          node contents={},
          ellipse,
          inner sep=0pt,
          outer sep=0pt,
          minimum width=2*\tqft@val{circle x radius},
          minimum height=2*\tqft@val{circle y radius},
          at={(\xpos pt,0)},
          name=-incoming boundary \k,
          /tikz/tqft/every skipped boundary component/.try,
          /tikz/tqft/every skipped incoming boundary component/.try,
          /tikz/tqft/skipped incoming boundary component \k/.try,
        ];
}%
\fi
      \path node also[pic alias=-incoming boundary] (-incoming boundary 1);
      \fi
      \ifnum\tqft@val{outgoing boundary components}>0\relax
\ifx\tqft@obdrylist\pgfutil@gobble
\xdef\tqft@obdrylist{1}
\else
\xdef\tqft@obdrylist{1,\tqft@obdrylist}
\fi
\foreach \k [evaluate=\k as \ok using int(\tqft@outgoing@end * (\tqft@val{outgoing boundary components} + 1) - \tqft@outgoing@dir * \k)] in \tqft@obdrylist {
  \xdef\tqft@robdrylist{\tqft@robdrylist,\ok}
}
      \foreach[
        evaluate=\k as \xpos using (\k-1+\tqft@val{offset})*\tqft@val{boundary separation}
      ] \k in \tqft@robdrylist {
  \node[
    transform shape,
          node contents={},
          ellipse,
          inner sep=0pt,
          outer sep=0pt,
          minimum width=2*\tqft@val{circle x radius},
          minimum height=2*\tqft@val{circle y radius},
          at={(\xpos pt,-\tqft@val{cobordism height})},
          name=-outgoing boundary \k,
          /tikz/tqft/every boundary component/.try,
          /tikz/tqft/every outgoing boundary component/.try,
          /tikz/tqft/outgoing boundary component \k/.try
        ];
}%
\ifx\tqft@cobdrylist\pgfutil@gobble
\else
\foreach \k[evaluate=\k as \ok using int(\tqft@outgoing@end * (\tqft@val{outgoing boundary components} + 1) - \tqft@outgoing@dir * \k)]
 in \tqft@cobdrylist {
  \xdef\tqft@rcobdrylist{\tqft@rcobdrylist,\ok}
}
      \foreach[
        evaluate=\k as \xpos using (\k-1+\tqft@val{offset})*\tqft@val{boundary separation}
      ] \k in \tqft@rcobdrylist {
  \node[
    transform shape,
          node contents={},
          ellipse,
          inner sep=0pt,
          outer sep=0pt,
          minimum width=2*\tqft@val{circle x radius},
          minimum height=2*\tqft@val{circle y radius},
          at={(\xpos pt,-\tqft@val{cobordism height})},
          name=-outgoing boundary \k,
          /tikz/tqft/every skipped boundary component/.try,
          /tikz/tqft/every skipped outgoing boundary component/.try,
          /tikz/tqft/skipped outgoing boundary component \k/.try
        ];
      }%
\fi
      \path node also[pic alias=-outgoing boundary] (-outgoing boundary 1);
      \fi
      \ifnum\tqft@val{incoming boundary components}>0\relax
      \foreach[evaluate=\k as \xpos using (\k-1)*\tqft@val{boundary separation}] \k in \tqft@ibdrylist {
        \path[
          /tikz/tqft/every lower boundary component/.try,
          /tikz/tqft/every incoming lower boundary component/.try,
          /tikz/tqft/incoming lower boundary component \k/.try
        ] (\xpos pt - \tqft@val{circle x radius},0) arc[start angle=\pgf@tqft@lower180,end angle=0, x radius=\tqft@val{circle x radius}, y radius =\tqft@val{circle y radius}];
      }%
      \fi
      \ifnum\tqft@val{outgoing boundary components}>0\relax
      \foreach[
        evaluate=\k as \xpos using (\k-1+\tqft@val{offset})*\tqft@val{boundary                   separation}
      ] \k in \tqft@robdrylist {
        \path[
          /tikz/tqft/every lower boundary component/.try,
          /tikz/tqft/every outgoing lower boundary component/.try,
          /tikz/tqft/outgoing lower boundary component \k/.try
        ] (\xpos pt - \tqft@val{circle x radius},-\tqft@val{cobordism height}) arc[start angle=\pgf@tqft@lower180,end angle=0, x radius=\tqft@val{circle x radius}, y radius =\tqft@val{circle y radius}];
        }%
      \fi
      \begin{scope}
      \path[overlay,clip] \tqft@gclip;
      \path[
        /tikz/tqft/cobordism/.try,
        pic actions,
        /tikz/tqft/cobordism outer path/.try,
      ] \tqft@fullpath;
      \end{scope}
\ifx\tqft@glist\pgfutil@gobble
\else
\foreach \tqft@gstyle/\tqft@gside/\tqft@gpath in \tqft@glist {
      \path[
        /tikz/tqft/cobordism/.try,
        pic actions,
        fill=none,
        shade=none,
        /tikz/tqft/cobordism edge/.try,
        /tikz/tqft/genus style/.try,
        /tikz/tqft/genus \tqft@gside/.try,
        /tikz/tqft/\tqft@gstyle/.try,
        /tikz/tqft/\tqft@gstyle\space\tqft@gside/.try,
      ] \tqft@gpath;
}
\fi
\ifx\tqft@blist\pgfutil@gobble
\else
\foreach \tqft@bstyle/\tqft@btype/\tqft@bpath in \tqft@blist {
      \path[
        /tikz/tqft/cobordism edge/.try,
        /tikz/tqft/cobordism outer edge/.try,
        /tikz/tqft/between \tqft@btype/.try,
        /tikz/tqft/\tqft@bstyle/.try,
      ] \tqft@bpath;
}
\fi
      \ifx\tqft@clist\pgfutil@gobble
      \else
      \foreach \name/\coord in \tqft@clist {
        \path \coord node[coordinate,node contents={},name=\name];
      }
      \fi
      \ifnum\tqft@val{incoming boundary components}>0\relax
      \foreach[evaluate=\k as \xpos using (\k-1)*\tqft@val{boundary separation}] \k in \tqft@ibdrylist {
        \path[
          /tikz/tqft/every upper boundary component/.try,
          /tikz/tqft/every incoming upper boundary component/.try,
          /tikz/tqft/incoming upper boundary component \k/.try
        ] (\xpos pt - \tqft@val{circle x radius},0) arc[start angle=\pgf@tqft@upper180,end angle=0, x radius=\tqft@val{circle x radius}, y radius =\tqft@val{circle y radius}];
      }
      \fi
      \ifnum\tqft@val{outgoing boundary components}>0\relax
      \foreach[
        evaluate=\k as \xpos using (\k-1+\tqft@val{offset})*\tqft@val{boundary                   separation}
      ] \k in \tqft@robdrylist {
        \path[
          /tikz/tqft/every upper boundary component/.try,
          /tikz/tqft/every outgoing upper boundary component/.try,
          /tikz/tqft/outgoing upper boundary component \k/.try
        ] (\xpos pt - \tqft@val{circle x radius},-\tqft@val{cobordism height}) arc[start angle=\pgf@tqft@upper180,end angle=0, x radius=\tqft@val{circle x radius}, y radius =\tqft@val{circle y radius}];
      }
      \fi
\end{scope}
  }
}

%% 
%% Copyright (C) 2011-2024 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  tqft_code.dtx,
%%                                  tqft.tex,
%% and the derived files            tqft_code.ins,
%%                                  tqft_code.pdf,
%%                                  tqft.pdf,
%%                                  tqft.sty, and
%%                                  tikzlibrarytqft.code.tex.
%% 
%%
%% End of file `tikzlibrarytqft.code.tex'.

